BriDe Arbitrager: Enhancing Arbitrage in Ethereum 2.0 via Bribery-enabled Delayed Block Production

The advent of Ethereum 2.0 has introduced significant changes, particularly the shift to Proof-of-Stake consensus. This change presents new opportunities and challenges for arbitrage. Amidst these changes, we introduce BriDe Arbitrager, a novel tool designed for Ethereum 2.0 that leverages Bribery-driven attacks to Delay block production and increase arbitrage gains. The main idea is to allow malicious proposers to delay block production by bribing validators/proposers, thereby gaining more time to identify arbitrage opportunities. Through analysing the bribery process, we design an adaptive bribery strategy. Additionally, we propose a Delayed Transaction Ordering Algorithm to leverage the delayed time to amplify arbitrage profits for malicious proposers. To ensure fairness and automate the bribery process, we design and implement a bribery smart contract and a bribery client. As a result, BriDe Arbitrager enables adversaries controlling a limited (< 1/4) fraction of the voting powers to delay block production via bribery and arbitrage more profit. Extensive experimental results based on Ethereum historical transactions demonstrate that BriDe Arbitrager yields an average of 8.66 ETH (16,442.23 USD) daily profits. Furthermore, our approach does not trigger any slashing mechanisms and remains effective even under Proposer Builder Separation and other potential mechanisms will be adopted by Ethereum.

==> data_version2/Feasibility_under_PBS_and_SSLE.tex <==
\section{Feasibility under PBS and SSLE}
\label{Feasibility under PBS and SSLE}
We explain the feasibility of Bribery-MEV Extractor under Proposer Builder Separation~\cite{pbs2021} (PBS) and Secret non-Single Leader Election~\cite{ssle2022} (SSLE) in this section.


\vspace{3pt}
\noindent
\textbf{Extended Threat Model. }
We extend our threat model of Section~\ref{threat model} to consider the PBS mechanism. The proposer finds the transaction strategy set using the DTOA in Section~\ref{sec:Delayed Arbitrage}. If there is available space left in the block, the proposer will select as many transactions with high gas prices and do not affect the liquidity pool involved in the strategy set from mempool. The proposer then broadcasts the transactions involved in the strategy set and the selected transactions from the mempool to the builders. Builders try to order the transactions selected by the proposer to maximize the MEV they can extract. Builders send the block and the corresponding bids back to the proposer. The proposer selects the block with the highest bid to obtain the corresponding bid.

% \vspace{3pt}
% \noindent
% \textbf{Feasibility under SSLE. }
% Recalling the bribery process, the adversary obtains the validators' client type, which is not hidden by SSLE, during communication with other validators. The bribery contract is activated when the adversary confirms that the number of bribery clients in the network meets the requirement~\ref{bribery_num1}. The validators deploying the bribery clients listen to the bribery message (event) through their clients and confirm whether the bribery fee satisfies the requirement~\ref{bribery_fee1}. If satisfied, they vote for the adversary's block. Finally, the bribee submits the corresponding proof to the bribery contract to withdraw the bribery fee. The bribery contract builds a broad trust bridge between the adversary and the rational validators without requiring the adversary to explicitly know which validators need to be bribed. Therefore, Bribery-MEV Extractor is still feasible under SSLE.

\vspace{3pt}
\noindent
\textbf{Feasibility under PBS. }
\begin{figure}[tp]
\centerline{\includegraphics[width=0.38 \textwidth]{results/PBS.png}}
\vspace{-10pt}
\caption{Profits under PBS.}
\vspace{-10pt}
\label{fig:pbs}
\end{figure}
The transactions that the proposer broadcasts to the builder are divided into three categories: the arbitrage transactions that we use to extract MEV (denoted $T_{arbitrage}$), the transactions selected by the transaction ordering (denoted $T_{others}$), and unrelated transactions (denoted $T_{unrelated}$). The builder with the highest bid only can profit from transactions in $T_{others}$ and $T_{unrelated}$. The order of the transactions in $T_{unrelated}$ will be irrelevant to DTOA's revenue because it does not affect liquidity pools involved in our arbitrage transactions. If the builder chooses to execute the transaction in $T_{others}$ before $T_{arbitrage}$, which is what we expect, we can get the expected revenue. If transactions in $T_{others}$ are executed after $T_{arbitrage}$, we may lose transaction fees because we are trading on a path without arbitrage opportunities. We predict that the execution order of the transactions in $T_{others}$ and $T_{arbitrage}$ will be random. We present our experimental results in Figure~\ref{fig:pbs}, which indicate that although the profit of Bribery-MEV Extractor decreases under PBS, it is still more profitable than honestly producing blocks.

==> data_version2/abstract.tex <==
\begin{abstract}
%\boldmath

The advent of Ethereum 2.0 has introduced significant changes, particularly the shift to Proof-of-Stake consensus. This change presents new opportunities and challenges for arbitrage. 
% concerning Maximal/Miner Extractable Value (MEV). 
Amidst these changes, we introduce BriDe Arbitrager, a novel tool designed for Ethereum 2.0 that leverages \underline{Bri}bery-driven attacks to \underline{De}lay block production and increase arbitrage gains. The main idea is to allow malicious proposers to 
delay block production
% extend their observation window 
by bribing validators/proposers, thereby gaining more time to identify profitable arbitrage opportunities. 
Through formalizing the bribery process, we design several bribery strategies for various scenarios.
% optimal bribery strategy that incurs the lowest cost. 
Additionally, we propose a Delayed Transaction Ordering Algorithm (DTOA)  to amplify the arbitrage profits for malicious proposers. To ensure fairness and automate the bribery process, we design and implement a bribery smart contract and a bribery client. As a result, BriDe Arbitrager effectively enables adversaries controlling $<1/4$ fraction of the voting powers to delay block production via bribery and arbitrage more profit. Extensive experimental results based on real Ethereum historical transactions demonstrate that BriDe Arbitrager yields an average of 8.66\,ETH (16,442.23\,USD) daily profits at a low cost. Furthermore, our approach does not trigger any slashing mechanisms and remains effective even under Proposer Builder Separation (PBS) and other potential future mechanisms proposed by Ethereum.


\end{abstract}
